Exploring the Advances in Identifying Useful Code Review Comments

Effective peer code review in collaborative software development necessitates useful reviewer comments and supportive automated tools. Code review comments are a central component of the Modern Code Review process in the industry and open-source development. Therefore, it is important to ensure these comments serve their purposes. This paper reflects the evolution of research on the usefulness of code review comments. It examines papers that define the usefulness of code review comments, mine and annotate datasets, study developers' perceptions, analyze factors from different aspects, and use machine learning classifiers to automatically predict the usefulness of code review comments. Finally, it discusses the open problems and challenges in recognizing useful code review comments for future research.

==> res/fig/corr.tex <==
\begin{figure}[t]%htbp
% \begin{figure}[h]%htbp
% \centerline{\includegraphics[width=0.9\linewidth]{dg_2.pdf}}
% \centerline{\includegraphics[trim={0 3.5cm 0 0},clip, width=0.99\linewidth]{res/fig/pdg_sera.pdf}}
\centerline{\includegraphics[trim={0 0.5cm 0 0.5cm},clip, width=0.9\linewidth]{res/fig/RHtest_text_fts_corr.png}}

\vspace{-2mm}
\caption{Correlation of Textual Features}
\label{fig_corrl}
\vspace{-4mm}
\end{figure}


==> res/fig/result_bar.tex <==
\begin{figure*}[h]%htbp
% \begin{figure}[h]%htbp
% \centerline{\includegraphics[width=0.9\linewidth]{dg_2.pdf}}
% \centerline{\includegraphics[trim={0 3.5cm 0 0},clip, width=0.99\linewidth]{res/fig/pdg_sera.pdf}}
\hspace{-7mm}
\centerline{\includegraphics[width=1.4\linewidth]{res/fig/result.png}}

% \vspace{-2mm}
\caption{CRAide Performance Comparison }
\label{fig_res}
% \vspace{-4mm}
\end{figure*}


==> res/fig/tool.tex <==
\begin{figure}[htbp]%htbp
% \begin{figure}[h]%htbp
% \centerline{\includegraphics[width=0.9\linewidth]{dg_2.pdf}}
% \centerline{\includegraphics[trim={0 3.5cm 0 0},clip, width=0.99\linewidth]{res/fig/pdg_sera.pdf}}
\centerline{\includegraphics[trim={0 3cm 0 3cm},clip, width=0.59\linewidth]{res/fig/tool.pdf}}

\vspace{-5mm}
\caption{CRAide (Tool) }
\label{fig_tool}
\vspace{-4mm}
\end{figure}


==> res/tbls/rough.tex <==
% \begin{table*}[h]
%     \centering
%     \begin{tabular}{c|c|cccccc}
%           \textbf{Decision Tree}  & 51.95 & 56.99 & 54.42 & 55.42 & 46.39 & 49.00 & 47.35 \\ \hline
%       \textbf{Random Forest}  & 53.86 & 58.00 & 61.10 & 59.28 & 48.22 & 45.03 & 46.25 \\ \hline
%                  \textbf{SVM}  & 54.65 & 57.71 & 73.94 & 61.68 & 52.43 & 30.56 & 31.05 \\ \hline
%       \textbf{Neural Network}  & 55.46 & 56.76 & 84.68 & 67.30 & 47.81 & 19.41 & 24.48 \\ \hline
%              \textbf{XGBoost}  & 54.33 & 57.60 & 66.78 & 61.66 & 48.73 & 39.06 & 43.06 \\ \hline
%  \textbf{Logistic Regression}  & 56.08 & 57.55 & 79.76 & 66.63 & 52.23 & 27.03 & 35.10 \\ \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}

==> res/tbls/tbl_matrix2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htbp]
% \renewcommand{\arraystretch}{1.3}
\centering
\small
\caption{Synthesis of Existing Works Regarding Usefulness of Code Review Comments}
\label{tbl_matrix}

\resizebox{0.8\linewidth}{!}{%
% \begin{tabular}{|p{0.1\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|}
%  \hline
%  & Bosu et al~\cite{bosu2015characteristics} &
% RevHelper~\cite{rahman2017predicting} &
% Efstathiou and Spinellis \cite{efstathiou2018code} &
% Meyers et al~\cite{meyers2018dataset} &
% CRA\cite{hasan2021usingCRA} 
%  \\ \hline
% Data Source (\crcs) &
%    from Microsoft &
%    X- Company &
%    Eclipse, Libre-Office, AOSP, OpenStack &
%     Chromium Conversations &
%     Samsung R\&D Bangladesh \\
% Factors as Input &
%   Textual, Activity &
%   Textual, Patch, Experience &
%   Textual, Patch &
%   Linguistic &
%   Textual, Patch, Activity, Experience \\
% Contribution &
%   Modeled Usefulness, Characterization, Prediction &
%   Feature Enhancement, Prediction, Dataset &
%   Preliminary work on Linguistics &
%   Dataset, Linguistic feature exploration &
%   Feature Enhancement, Prediction \\
% Evaluation Metric &
%   Accuracy, Precision, Recall &
%   Accuracy, Precision, Recall, F1 &
%   Distribution &
%   Precision, Recall, F1, AUC &
%   Accuracy, Precision, Recall, F1\\ \hline
% \end{tabular}%
\begin{tabular}
% {@{}lllll@{}}
{|p{0.15\linewidth}|p{0.10\linewidth}|p{0.10\linewidth}|p{0.15\linewidth}|p{0.10\linewidth}|p{0.10\linewidth}|}
\hline
\textbf{Seed Papers}
 & \textbf{Data Source}
 & \textbf{Factors as Input} 
 & \textbf{Contribution}
 & \textbf{Evaluation Metric}  
 & \textbf{Validation} \\ 
 \hline
 
Pangsakulyanont et al.~\cite{pangsakulyanont2014assessing} 
& Qt project 
& commit-message 
& Modeled Usefulness & Accuracy, Precision, Recall & 300x10-fold \\  \hline

Bosu et al.~\cite{bosu2015characteristics}
&  Microsoft 
& Textual, Activity 
& {Modeled Usefulness, Characterization, Prediction} 
& Accuracy, Precision, Recall & 100x10-fold \\ 
\hline

Rahman et al.~\cite{rahman2017predicting} 
& Anonymous Company 
&  Textual, Patch, Experience 
&  Feature Enhancement, Prediction, Dataset 
&  Accuracy, Precision, Recall, F1 & 1x10-fold \\ 
  \hline

Efstathiou \& Spinellis \cite{efstathiou2018code}    
&  Eclipse, AOSP, Libre Office, OpenStack 
& Textual, Patch 
& Preliminary work on Linguistics 
& Distribution                & n/a \\ 
\hline

Meyers et al.~\cite{meyers2018dataset} 
& Chromium Conversations 
& Linguistic 
& Dataset, Linguistic feature exploration 
& Precision, Recall, F1 , AUC & 10x10-fold \\ 
\hline
  
Hasan et al.~\cite{hasan2021usingCRA} 
&   Samsung R\&D Bangladesh 
&  Textual, Patch, Activity, Experience 
& Feature Enhancement, Prediction 
& Accuracy, Precision, Recall, F1 & 20x10-fold \\  
\hline
  
\end{tabular}
}
\end{table*}
